InScope: A New Real-world 3D Infrastructure-side Collaborative Perception Dataset for Open Traffic Scenarios

Perception systems of autonomous vehicles are susceptible to occlusion, especially when examined from a vehicle-centric perspective. Such occlusion can lead to overlooked object detections, e.g., larger vehicles such as trucks or buses may create blind spots where cyclists or pedestrians could be obscured, accentuating the safety concerns associated with such perception system limitations. To mitigate these challenges, the vehicle-to-everything (V2X) paradigm suggests employing an infrastructure-side perception system (IPS) to complement autonomous vehicles with a broader perceptual scope. Nevertheless, the scarcity of real-world 3D infrastructure-side datasets constrains the advancement of V2X technologies. To bridge these gaps, this paper introduces a new 3D infrastructure-side collaborative perception dataset, abbreviated as inscope. Notably, InScope is the first dataset dedicated to addressing occlusion challenges by strategically deploying multiple-position Light Detection and Ranging (LiDAR) systems on the infrastructure side. Specifically, InScope encapsulates a 20-day capture duration with 303 tracking trajectories and 187,787 3D bounding boxes annotated by experts. Through analysis of benchmarks, four different benchmarks are presented for open traffic scenarios, including collaborative 3D object detection, multisource data fusion, data domain transfer, and 3D multiobject tracking tasks. Additionally, a new metric is designed to quantify the impact of occlusion, facilitating the evaluation of detection degradation ratios among various algorithms. The Experimental findings showcase the enhanced performance of leveraging InScope to assist in detecting and tracking 3D multiobjects in real-world scenarios, particularly in tracking obscured, small, and distant objects. The dataset and benchmarks are available at https://github.com/xf-zh/InScope.

==> tables/old_table1.tex <==

\begin{table*}
    \caption{\textbf{Dataset comparison.} 2D and 3D represent the image and point cloud, respectively. V2V: Vehicle cooperative system, I2I: Infrastructure cooperative system, V2X: Vehicle-infrastructure cooperative system. ``Real/Sim.'' indicates the datasets are collected in the real or simulated world. 
    % ``TA'': Trajectory Annotation. 
    ``BSS'': Blind Spot Supplementation. ``QAC'': Quantitatively Assess the Anti-occlusion Detection Capabilities. 
    % ``NBs'': Numbers of Benchmarks.}
    }
    \centering
    \footnotesize
    \begin{tabular}{cccccccccc}
    \toprule
    Dataset & View  & Real/Sim & Year  & \multicolumn{1}{l}{Point Clouds} & 3D Boxes & Trajectory & BSS & QAC & Benchmarks\\
    \midrule
    KITTI \cite{geiger2012we}                   & Single-vehicle & Real  & 2012  & 15k   & 200k  & \ding{51} & \ding{55}  & \ding{55} & 5 \\
    ApolloScape \cite{huang2018apolloscape}     & Single-vehicle & Real  & 2018  & -     & 70k   & \ding{51} & \ding{55}  & \ding{55} & 5 \\
    nuScenes \cite{caesar2020nuscenes}          & Single-vehicle & Real  & 2020  & 400k  & 1.4M  & \ding{51} & \ding{55}  & \ding{55} & 2 \\
    Waymo \cite{sun2020scalability}             & Single-vehicle & Real  & 2020  & 200k  & 12M   & \ding{51} & \ding{55}  & \ding{55} & 2 \\
    ONCE  \cite{mao2021one}                     & Single-vehicle & Real  & 2021  & 1M    & 417k  & \ding{55} & \ding{55}  & \ding{55} & 4 \\
    V2V4Real \cite{xu2023v2v4real}              &      V2V       & Real  & 2023  & 20k   & 240K  & \ding{51} & \ding{51}  & \ding{55} & 3 \\
    \midrule
    V2X-Sim \cite{li2022v2x}                    &      V2X       & Sim.   & 2022  & 10k   & 26.6k & \ding{51} & \ding{51}  & \ding{55} & 4 \\
    V2X-Seq/Perception \cite{yu2023v2x}         &      V2X       & Real  & 2023  & 15k   & 12k   & \ding{51} & \ding{51}  & \ding{55} & 2 \\
    \midrule
    NGSIM \cite{NGSIM}                          & Infrastructure & Sim.   & 2016  & -     & -     & \ding{51} & \ding{55}  & \ding{55} & 7 \\
    WIBAM \cite{WIBAM}                          & Infrastructure & Real  & 2021  & -    & -     & \ding{55} & \ding{55}  & \ding{55} & 1 \\
    DAIR-V2X-I \cite{yu2022dair}                & Infrastructure & Real  & 2022  & 10k   & 493k  & \ding{55} & \ding{55}  & \ding{55} & 1 \\
    RCooper-Corridor \cite{hao2024rcooper}      &I2I-Corridor     & Real  & 2024  & 11k    & 53k   & \ding{51} & \ding{51}  & \ding{55} & 2 \\
    RCooper-Intersection \cite{hao2024rcooper}  &I2I-Intersection     & Real  & 2024  & 2k    & 43k   & \ding{51} & \ding{51}  & \ding{55} & 2\\
    \midrule
    \textbf{InScope} (ours)                     & I2I-Intersection           & Real  & 2024  & 21k   & 188k  & \ding{51} & \ding{51}  & \ding{51} & 4\\
    \bottomrule
    \end{tabular}
  \label{tab:dataset}
\end{table*}
